SPICED: Syntactical Bug and Trojan Pattern Identification in A/MS Circuits using LLM-Enhanced Detection

Analog and mixed-signal (A/MS) integrated circuits (ICs) are crucial in modern electronics, playing key roles in signal processing, amplification, sensing, and power management. Many IC companies outsource manufacturing to third-party foundries, creating security risks such as stealthy analog Trojans. Traditional detection methods, including embedding circuit watermarks or conducting hardware-based monitoring, often impose significant area and power overheads, and may not effectively identify all types of Trojans. To address these shortcomings, we propose SPICED, a Large Language Model (LLM)-based framework that operates within the software domain, eliminating the need for hardware modifications for Trojan detection and localization. This is the first work using LLM-aided techniques for detecting and localizing syntactical bugs and analog Trojans in circuit netlists, requiring no explicit training and incurring zero area overhead. Our framework employs chain-of-thought reasoning and few-shot examples to teach anomaly detection rules to LLMs. With the proposed method, we achieve an average Trojan coverage of 93.32% and an average true positive rate of 93.4% in identifying Trojan-impacted nodes for the evaluated analog benchmark circuits. These experimental results validate the effectiveness of LLMs in detecting and locating both syntactical bugs and Trojans within analog netlists.

==> Add.tex <==
produce a structured output of single/multiple bugs, and rectify the bug in the code.

what prompts do i try to give structured format?

1)create a bug detection report. 

2)pass detection report as prompt+old netlist-->make model correct the error i.e. give the correct netlist.
3) iterate to get a clean report. check for syntax errors.

Functional bugs:

action taken to correct the line: remove the lines or edit the lines (if Trojan involves changing parameter values) based on LLM feedback.

Trojan is subset of bug for design-time attacks

Note that this a  form of functional bug, which means that LLM will have to understand from the prompt itself.

Report:

LLM2-13b takes 1m 36 s for inferencing on A100 GPU.


point out bugs and giving the confidence score.

also give llm a trojan-free circuit. 


References: 

1. Externally activated Trojans. https://static.googleusercontent.com/media/research.google.com/en//pubs/archive/37398.pdf

Tasks: 

1. Complete all bug detection experiments.
2. Add the prompt figures to the paper.
3. Prepare the methodology for Trojan detection
4. Prepare a CoT for teaching unsupervised learning to LLM.


Supervised problem. convenient and interpretable.


==> Experiments_to_be_done.tex <==
1. Ask LLM to resolve bug i.e., all bugs identified?
2. Trojan mitigation is challenging

==> To_be_added.tex <==
1. LLAMA 2 and GPT 4 carbon footprint overhead

2. Difficulty level of Trojan, and accuracy of LLMs in detecting the Trojan.


**Importance of LLM:

LLMs can effectively parse the log file, and understand the current and voltage behavior for all the nodes. it can also learn what is the desired voltage range where circuit should work. LLMs can be taught to follow rules with CoT.

Methodology:

We are using Chain of thought accompanied by few-shot learning to teach LLM an unsupervised method to identify Trojan impacted nodes. 

When testing a new buggy netlist with unknown bug locations, you rely entirely on the LLM to identify and resolve all the bugs. Since the exact bug locations are unknown, the SPICE syntax rules cannot be updated in this context. The process would then focus on the LLM's ability to comprehensively detect and address bugs based on the existing rules and its learned capabilities.

Flow:

You are given a SPICE netlist of a circuit, the voltage and current simulation logs of the netlist, and the desired output voltage specifications. Given these information, you will follow a set of specific rules to identify Trojan-impacted nodes of the circuit. Assume that the output voltage of the circuit should be less than Vout.

Rule 1: Analyze voltage behavior of circuit nodes

1.1. Check the output voltage, and compare with the desired specification, for the entire input voltage range.
1.2. If the output voltage is within the desired specification for all the input voltages, classify the circuit as Trojan-free.
1.3. If the output voltage is outside the desired specification, find and list all the input voltages where where the output voltage is outside the desired specification. 

1.4. Now you have the list of input voltages. For each input voltage, check the corresponding node voltages from the simulation log. 
pick a node and check its voltages for the output where it does not meet spec.

check trend in anomalous window and non anomalous node.

2) check across nodes to decide for anomaly. check trends of all nodes. across all nodes, llm will study ckt behavior.

anomaly detection in 2D. one across input voltages, one across nodes. 




Comparison:

1. few-shot learning without rules
2. Apply intersection (voltage)
3. current decreases significantly, which means that node is not trojan.
4. 2+3
5. only rules (without few-shot)

Todays tasks:

1. add the bug results.
2. Finish the remaining tasks for few-shot+rules.


voltage deviation define, add unit.

fig 3 mention current analysis and voltage analysis
